Improving Multi-hop Logical Reasoning in Knowledge Graphs with Context-Aware Query Representation Learning

Multi-hop logical reasoning on knowledge graphs is a pivotal task in natural language processing, with numerous approaches aiming to answer First-Order Logic (FOL) queries. Recent geometry (e.g., box, cone) and probability (e.g., beta distribution)-based methodologies have effectively addressed complex FOL queries. However, a common challenge across these methods lies in determining accurate geometric bounds or probability parameters for these queries. The challenge arises because existing methods rely on linear sequential operations within their computation graphs, overlooking the logical structure of the query and the relation-induced information that can be gleaned from the relations of the query, which we call the context of the query. To address the problem, we propose a model-agnostic methodology that enhances the effectiveness of existing multi-hop logical reasoning approaches by fully integrating the context of the FOL query graph. Our approach distinctively discerns (1) the structural context inherent to the query structure and (2) the relation-induced context unique to each node in the query graph as delineated in the corresponding knowledge graph. This dual-context paradigm helps nodes within a query graph attain refined internal representations throughout the multi-hop reasoning steps. Through experiments on two datasets, our method consistently enhances the three multi-hop reasoning foundation models, achieving performance improvements of up to 19.5%. Our code is available at https://github.com/kjh9503/caqr.

==> introduction_backup.tex <==
\section{Introduction}\label{introduction}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{fig/figure1.png}
    \caption{Existing models convert the FOL query into a computation graph, and then predict the correct answer through the embedding (or probability space) of the answer node (A) by sequential inference from the anchor node. In this example, the existing methods contain wrong answers such as attractions, rivers, and mountains because the candidates held by the variable node (V) in the inference process are only influenced by the anchor node. However, our  approach uses global and local contexts to find a more accurate embedding of V, which allows us to predict better answers.}
    \vspace{-2mm}
    \label{fig:figure1}
\end{figure}
\hjc{the definition of knowledge graph is not really required in NLP conferences, I believe. Also, the current definition seems too ...} In recent years, real-world knowledge has been more actively incorporated into large-scale graph data structures, known as knowledge graphs (KGs) \cite{sinha2015overview, vrandevcic2014wikidata}. KGs are composed of a set of entities and relationships between them, providing richer and less ambiguous knowledge representations for various reasoning tasks \hjc{citations}.
Multi-hop logical reasoning on KGs aims to predict answer entities from First-order Logic (FOL) queries on large-scale incomplete KGs \hjc{does multi-hop logical reasoning always involve FOL?}. \hjc{what is FOL?} Each FOL query can be mapped one-to-one to a dependency graph, comprising multiple variables, conjunctions, and existential quantification operators, effectively representing natural language questions.
% are structured data rather than natural language questions and are obtained from the KG in the form of 14 predefined query types, such as Query Graph 1, 2 in Figure~\ref{fig:figure1}. 
% These queries are represented in the form of query graphs.}
% which are typically formulated using First-Order Logic (FOL) connectives,} including existential quantification ($\exists$), conjunction ($\wedge$), disjunction ($\lor$), and negation ($\neg$)$. A prevalent approach~\cite{gqe} translates these queries into computation graphs, where nodes represent entities (either constants or variables) and edges correspond to predicates and logical operations. This representation simplifies the traversal of KG paths via the computation graph, enabling the extraction of answers for a given query. 
% Nonetheless, challenges emerge due to the inherent incompleteness and noise in large-scale KGs. Such complexities often cause explicit query mechanisms to inconsistently retrieve accurate answers, particularly when grappling with intricate query structures and gaps in the graph data. 
% Each query corresponds to a query graph represented as a Directed Acyclic Graph (DAG). An example query graph is visualized in Figure~\ref{query_types}. 
While traditional multi-hop reasoning approaches~\cite{dalvi2007efficient} struggle with the inherent incompleteness and noise in large-scale KGs, embedding-based multi-hop logical reasoning models have recently been proposed and achieved significant enhancement in prediction. These models predict the answer to queries on latent embedding spaces, such as point~\cite{gqe}, box~\cite{q2b}, and cone~\cite{cone}), or by employing probability distributions like the beta distribution~\cite{betae}. In these models, entities and queries are embedded into a corresponding latent space such that entities answering a query are close to the embedding of the query.
% a given query \MG{in the corresponding latent space} using neural networks and find the nearest entities to the query embedding for the prediction.
% , based on a predetermined order for each query type, to answer the complex queries from the KGs.
%These methodologies embed a given query by employing neural networks to implement relational projection or intersection operation, based on a predetermined order for each query type,  to answer the query.
%Similar to prior methods, these embedding techniques also convert the input query into a corresponding computation graph. The graph is then embedded using neural operators to predict answer entities.
% To obtain answers to complex queries from the knowledge graph (KG), they embed a given query using neural network to facilitate logical operators.

However, a significant challenge persists in determining accurate geometric bounds or probability parameters for these queries. Prior embedding-based methods (e.g., Q2B~\cite{q2b}, Beta embedding~\cite{betae}, and ConE~\cite{cone}) rely on linear sequential operations regardless of different query types, overlooking the context of the input query. In other words, the existing query embedding approaches construct the embedding of each branch (i.e., edge) independently and sequentially, which fails to capture both the global and local context of the query. 

To address these challenges, we propose a logical query embedding technique that captures both the \textit{global structural context} of the entire query structure and the \textit{local relation-induced context} specific to each node in the query graph, induced from the corresponding KG. This approach aims to enhance existing multi-hop logical reasoning methods, such as Q2B, Beta embedding, and ConE. First, we employ position and role information from the query graph to generate a summarization table that represents the query's \textit{global structural context}. Furthermore, to capture the \textit{local relation-induced context}, we utilize entities from the KG, taking into account relations connected to each node in the query graph. These two contexts collectively refine node representations during logical reasoning steps, enabling the determination of more precise geometric bounds or probability parameters. For example, as in Figure \ref{fig:figure1}, the existing methods produce errors, such as incorrectly identifying attractions, rivers, and mountains, due to the variable node (V) in the inference process being influenced solely by the anchor node. In contrast, this paper utilizes both global and local contexts to achieve a more precise embedding of V, thereby facilitating more accurate predictions. The global context encodes the positional or role-like information of the query nodes. Meanwhile, the local context offers additional insights from the triples in KGs, derived from nearby relations such as $LocatedIn^{-1}$ and $Hold$. In evaluation, experimental results on two datasets show that our method consistently enhances three recent multi-hop reasoning models, achieving improvements on query reasoning tasks up to 19.5\%.



% For example, as in the upper side of Figure \ref{fig:figure1}, the global structural context could indicate whether a query seeks a ``factual answer" or ``serial reasoning." 

% Moreover, existing methods' multi-hop logical reasoning steps do not leverage the \textit{local contextual information} \textcolor{red}{that can be extracted from the KG using neighboring relations of the node.}%{such as neighboring relations of each node in the query graph and their associated nodes in the KG.} 


% The information contained in a query can be explained as (1) global structural information of the query graph, and (2) localized node information that is induced by relation comprising query graph.
% % However, existing methodologies overlook this information inherent in the query graph, as they solely rely on sequential query execution to obtain query embeddings based on the computation graph. Therefore, to exploit the structural information and relation-inducing information present in the query graph, 
% In order to enable existing query embedding methodologies to sufficiently incorporate both the global structural information of the query graph and the localized information of individual nodes that can be inferred from relations, which enhances the reasoning capability, we propose a novel methodology \mname{}. To the best of our knowledge, our methodology represents the first model that concurrently integrates the structural global information inherent in the query graph and the localized information specific to individual nodes into the query embedding methodology. The contributions of our model are as follows:
% \begin{itemize}
%     \item \mname{} utilizes the global structural information of the query graph for enhancing multi-hop reasoning capability.
%     \item \mname{} extracts localized information from the neighboring relations of nodes composing the query graph and employs it for reasoning.
%     \item \mname{} is a model-agnostic methodology, which can be applied to various query embedding-based multi-hop reasoning models.
% \end{itemize}



% =======

% Multi-hop reasoning over KG is a task of finding answers to complex queries on the knowledge graph, which has recently been in the limelight with the development of Artificial Intelligence. It enables more sophisticated applications in various domains such as recommendation systems, question answering, and semantic search~\cite{nrn}. A knowledge graph constitutes a collection of $(h, r, t)$, triples, where $h$ and $t$ represent the head and tail entities respectively, and $r$ denotes the relation. Queries for reasoning over KG span from simple tasks like predicting the tail given the head and relation, to more intricate tasks such as predicting entities that satisfy tail of three sets of head and relation pairs.
% The query for reasoning is in the form of first-order logic (FOL), encompassing existential quantification ($\exists$), conjunction ($\wedge)$, disjunction ($\lor$), and negation ($\neg$). Each query corresponds to a query graph represented as a Directed Acyclic Graph (DAG). The types of queries addressed herein are documented in the Figure~\ref{query_types}.
% To deal with the multi-hop reasoning task, recent studies have proposed to embed the query itself, entities and relations, into the same low-dimensional space. In particular, a line of research has achieved notable progress that employs geometric representations (points~\cite{gqe}, boxes~\cite{q2b} and cones~\cite{cone}) or probability distributions (beta~\cite{betae} and gamma~\cite{gammae}) to represent the query, its entities and relations. 
% These query embedding methodologies transform a given query into a corresponding computation graph and embed the query employing the logical operators defined by the model according to this computation graph~\cite{traversing}.



% Therefore, $r_1(e_1, A)$ and $r_1(e_1, A)$ should return different representations (i.e.,  answering v.s., clarifying the queries). 


%This process of obtaining query embedding by applying logical operators based on the computation graph is referred to as \textit{query execution}. \q{WHAT ARE QUERY TYPES?}

% figure here
% \begin{figure}[t]
%      \centering
%      \begin{subfigure}[b]{0.3\textwidth, height=7cm}
%          \includegraphics[width=\textwidth]{fig/figure_1a.png}
%          \caption{An example of structure-possessing information inherent in query graph.}
%          \label{meta_structural_info}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{fig/figure_1b.png}
%          \caption{An example of relation-possessing context information inherent in query graph.}
%          \label{meta_semantic_info}
%      \end{subfigure}

% \caption{Two examples of information that need to be considered when obtaining query embedding. The figure (a) illustrates the structural information obtainable from the query graph. , the representations of A and V should differ. However, traditional query embedding is generated sequentially, resulting in the same representation. This also holds true when examined from the perspective of the query graph. The domain of node A varies significantly, with \textit{University} when the connected edge is \textit{Tenure(Enrico Fermi, A)}, and with \textit{country} when it is \textit{ParticipatingCountry(2012 Olympics, A)}. Consequently, the node A should have different representations for \textit{Contains(Europe, A)} in Query Graph 1 and Query Graph 2. The figure (b) demonstrates that hints for the nodes in the query can be obtained from the neighbor relations. Leveraging the relations as intermediaries, we can obtain rough understanding of information pertaining to node V through the KG.}
% \label{figure1}
% \end{figure}





% \textcolor{blue}{However, these methodologies embed entities and relations only considering the corresponding branch(edge) even though there are multiple branches on a single query structure.} \todo{NEED TO CLARIFY WHAT IS BRANCH HERE.} Therefore they fail to incorporate information inherent in the query graph. As a result, such methodologies do not take into account the situation in which the same entity or branch should have different representations by this information.

%Then, they use the intersection operator to obtain the intersection of the already constructed branch embeddings. 
% \sout{In other words, since the intersection operation calculates the intersection of the pre-existing branches, not providing  opportunity for branch embeddings to incorporate the information from the adjacent branches information.} 
% \textcolor{blue}{In other words, the intersection operation computes the common elements among existing branches, but it doesn't allow each branch embedding to include information from adjacent branches.} \hp{The previous sentences sound not clear.} To overcome the limitation of sequentiality inherent in conventional query embedding methodologies, we provide structural and contextual information of the query graph during the branch embedding construction phase.


%In the case of 1p query, the answer node of the branch beginning with \textit{Official Website} can include all entities that have \textit{websites} as candidates. However, for 2i, only entities that have \textit{revenue}(e.g., \textit{companies}) can be considered as candidate answers. 
% For instance, the right figure of Figure~\ref{fig:figure1} illustrates the structural information of the query graph that cannot be captured using the conventional query embedding approach. 
% Considering a query graph as a subgraph of the KG, subgraph 1 and subgraph 2 have different structures, leading to distinct representations between node A in subgraph 1 and node V in subgraph 2.
% \textcolor{blue}{Due to the dissimilarities in their connectivity, node A in subgraph 1 and node V in subgraph 2 need to have separate representations.}
% \hp{why this sould be distinct?} However, the existing query embedding methodologies sequentially construct embedding from the anchor node, resulting in the same representation for node A and node V. Hence, there is a need to consider the structural information of the query graph when constructing query embedding. This holds true even from the perspective of the query graph, not just subgraph. The lower figure of Figure~\ref{meta_structural_info} presents an example where, even for the same branch, it should be expressed differently depending on the structure of the query graph. Node A is constrained to the \textit{Country} domain by the branch \textit{ParticipatingCountries(2012 Olympics, A)} in query graph 1, but in query graph 2, it is constrained to the \textit{University} domain by the branch \textit{Tenure(Enrico Fermi, A')}, indicating that \textit{Contains(Europe, A)} should have different representations based on the structure of query graph.

% For instance, the upper figure of Figure~\ref{meta_structural_info} illustrates the necessity of incorporating structural information of the query graph into query embedding. The left figure (Query Graph 1) represents the query \textit{'All the things that is contained in Europe'}. Thus, all the entities that is in \textit{Europe} can be candidates for node A, such as \textit{University of London, Republic of Ireland, Italy, Danube}. However, the right figure (Query Graph 2) signifies the query \textit{'All the entities contained in Europe that that has participated in 2012 Olympic'}, and the edge (branch) indicating \textit{Participating Country} of the \textit{2012 Olympic} narrows down the scope of node A to entities that is categorized into \textit{country} (e.g., Republic of Ireland, Italy). \q{BUT IT CAN ALREADY BE DEALT WITH BY INTERSECTION OPERATOR.} 
% In addition, the lower figure in Figure~\ref{meta_structural_info} provides another example of how the multi-hop reasoning process can be influenced by the the structure of the query graph. The left figure (Query Graph 3) indicates the query \textit{'Region that contains Rotterdam'}. The candidate entities for A of the branch \textit{$Contained^{-1}$(Rotterdam, A)} include all the entities that contains \textit{Rotterdam} geographically. On the other hand, the right figure (Query Graph 4) represents the query \textit{'Olympic in which country containing rotterdam geographically participated'}. Even if it has the same branch as in the Query Graph 3, the candidates for the node V are reduced compared to those in Query Graph 3 due to the additional relation surrounding the node V. Thus, \textit{$Contains^{-1}$(Rotterdam, A)} and \textit{$Contains^{-1}$(Rotterdam, V)} requires different representations because additional information is provided associated with the node V. For these reasons, the answer nodes or variable nodes of the query graph should be distinguishable based on their structure (e.g., having one more incoming edge or one more outgoing edge), even if they are the same branch. Furthermore, when considering the query graph as a subgraph of the KG, the Query Graph 1 and Query Graph 2 posses distinct structures. As a result, node A should have different embeddings in the two graphs.

% \begin{figure*}
%      \centering
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, height=3.5cm]{emnlp2023-latex/fig/figure_1a.png}
%          \vspace{-4mm}
%          \caption{An example of structure-possessing meta information.}
%          \label{meta_structural_info}
%      \end{subfigure}
%      \hspace{10mm}
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, height=4cm]{emnlp2023-latex/fig/figure_1b.png}
%          \vspace{-4mm}
%          \caption{An example of relation-possessing meta information}
%          \label{meta_semantic_info}
%      \end{subfigure}

% \caption{Two types of meta information from query graph. The upper figure of (a) illustrates that the embedding of the same branch should vary depending on the type of the query. In the case of 1p query, the answer node of the branch beginning with \textit{Official Website} can include all entities that have \textit{websites} as candidates. However, for 2i, only entities that have \textit{revenue}(e.g., \textit{companies}) can be considered as candidate answers. The figure (b) shows that neighbor relations provide hints about the identity of the variable node.}
% \label{figure1}
% \end{figure*}
